Structural-RNN: Deep Learning on Spatio-Temporal Graphs

Deep Recurrent Neural Network architectures, though remarkably capable at modeling sequences, lack an intuitive high-level spatio-temporal structure. That is while many problems in computer vision inherently have an underlying high-level structure and can benefit from it. Spatio-temporal graphs are a popular tool for imposing such high-level intuitions in the formulation of real world problems. In this paper, we propose an approach for combining the power of high-level spatio-temporal graphs and sequence learning success of Recurrent Neural Networks~(RNNs). We develop a scalable method for casting an arbitrary spatio-temporal graph as a rich RNN mixture that is feedforward, fully differentiable, and jointly trainable. The proposed method is generic and principled as it can be used for transforming any spatio-temporal graph through employing a certain set of well defined steps. The evaluations of the proposed approach on a diverse set of problems, ranging from modeling human motion to object interactions, shows improvement over the state-of-the-art with a large margin. We expect this method to empower new approaches to problem formulation through high-level spatio-temporal graphs and Recurrent Neural Networks.

==> experiment_backup.tex <==
\iffalse
In this experiment we study S-RNN for modeling and forecasting human motion from
motion capture (``mocap'') data. This is a challenging problem because human
skeleton is high-dimensional with 54 degrees of freedom, and different parts of
the skeleton interact in a complex manner during an activity. For example the
motion of the two human legs strongly correlates while walking and their
interaction should be modeled differently than the interaction between the two
arms. Furthermore the spine of human skeleton interacts with both legs and arms
in order to maintain a physically realizable posture. We represent such
part-based interactions between different body parts with a st-graph as shown in
Figure~\ref{fig:stgraph}\rc{a}. According to the st-graph, the spine interact
with all the body parts, and the arms and legs interact with each other. Our
goal is to learn an S-RNN architecture based on this st-graph for modeling the
human motion. We should note that our technique applies equally to other
representations of human motions with st-graphs, e.g. a fully connected graph.
Therefore we give flexibility to practitioners to design their
``\textit{favourite}'' st-graph based on their intuition about the application.
% Such part-based interactions between body parts can be represented with a
% st-graph. In this experiment we capture it with the st-graph shown in
% Figure~\ref{fig:stgraph}(a). 

Our goal is to learn a model of human motion from motion capture data. We
therefore train our S-RNN architecture to predict the mocap skeleton at time
$t+1$ (next frame) given the skeleton at time $t$ (current frame). At test time
we feed the architecture with a set of seed mocap frames and forecast the future
motion. We use the H3.6m motion capture data set~\citep{H36m} and compare
ourselves with the recent results from Fragkiadaki et al.~\citep{Fragkiadaki15}
on the same data set. 

\noindent \textbf{Structural-RNN for human motion.} Our S-RNN architecture for
modeling human motion follows the st-graph shown in
Figure~\ref{fig:stgraphexp}\rc{a}. Our architecture have three nodeRNNs, one for
each type of body part (spine, arm, and leg), four edgeRNNs for modeling
interactions between body parts (spine-arm, arm-arm, spine-leg, and leg-leg),
and three edgeRNNs for temporal connections between the body parts. Following
the definitions in Section~\ref{subsec:srnn}, the nodeRNNs and edgeRNNs are
connected to form the S-RNN architecture. 

Since the input into our architecture are raw skeleton values, our edgeRNNs
(nodeRNNs) include fully-connected encoders (decoders) for representation
learning. Using encoders and decoders with RNNs have been shown to work well on
several problems which start with raw data~\citep{Hannun14,Fragkiadaki15}. The
architecture of the edgeRNNs we use is FC(256)-FC(256)-LSTM(512) with skip input
and output connections~\citep{Graves13}. The number inside parenthesis is the
size of layer. Our nodeRNNs includes an LSTM followed by fully-connected
decoding layers to predict the next mocap frame:
LSTM(512)-FC(256)-FC(100)-FC($\cdot$). The output layer of nodeRNNs predict the
mocap values of a body part. The outputs of nodeRNNs are concatenated to
generate the complete skeleton. The node features in st-graph are raw joint
values expressed as exponential map~\citep{Fragkiadaki15}, and edge features are
concatenation of node features.  \todo{See supplementary for a detailed
architecture of the structural-RNN for human motion.}



\noindent \textbf{Evaluation setup.} We compare S-RNN with the recent work from
Fragkiadaki et al.~\citep{Fragkiadaki15} which demonstrated state-of-the-art
results on motion forecasting. Fragkiadaki et al.~\citep{Fragkiadaki15} proposed
an encoder-RNN-decoder (ERD) architecture for modeling human motion. We
reproduced their ERD architecture, and the 3 layer LSTM architecture (size 1000
each layer) which they use as a baseline.\footnote{Their implementation or
models were not available as of Oct. 2015} In order to evaluate, we seed the
architectures with several mocap frames and then forecast the future frames.  We
use H3.6m motion capture data set (down sampled by two) and train on 6 subjects
and test on hold-out subject S5. We consider four human activity: walking,
eating, smoking, and discussion. Since human motion is stochastic, a
\textit{good} model of human motion should generate plausible human-like motion
in the distant future while staying close to the ground-truth in the near
future. Motion forecasting becomes specially challenging on activities with
\textit{aperiodic} human motion such as eating, smoking, and discussion. 




Our evaluation goes beyond Fragkiadaki et al.~\citep{Fragkiadaki15} in three
important ways: (i) We visualize and present quantitative results on challenging
aperiodic activities such as eating, smoking, etc. Fragkiadaki et
al.~\citep{Fragkiadaki15} presented results only on periodic walking motion;
(ii) We forecast human motion for almost twice longer than Fragkiadaki et
al.~\citep{Fragkiadaki15}. Such long-term forecasting is challenging for
aperiodic activities where a good model of human motion should generate
plausible human-like motion in the distant future; and finally (iii) In
Section~\ref{sec:visualize} we visualize the memory cells of S-RNN and show they
learn certain semantic concepts. 


\noindent \textbf{Qualitative results on motion forecasting.}
Figure~\ref{fig:eating_videos} shows motion forecasting 1000ms into the future
on eating activity, where the subject drinks while walking. The seed mocap frame
is shown with blue color and the forecasted frames are shown in green. S-RNN
models the human motion well and generates most realistic forecasts. It stays
close to the ground truth early in time and generates smooth realistic motion in
the distant future. LSTM-3LR on the other hand also generates plausible human
like motion however we observe that (on many test examples) it converges to the
mean motion of a walking human. For the same reason LSTM-3LR forecasting results
in Figure~\ref{fig:eating_videos} differ from the ground truth since the
beginning. The motion generated by ERD~\citep{Fragkiadaki15} stays close to the
ground truth early in time but it drifts away to non-human like motion in the
distant future as shown in Figure~\ref{fig:eating_videos}. We observed this
behaviour of ERD mostly on aperiodic activities. Furthermore the quality of
motion generated by ERD was not smooth (as also noted by~\citep{Fragkiadaki15}).
When forecasting long-term on aperiodic activities, both ERD and LSTM-3LR fails
to generate human-like motion on many test example. . 

The good performance of S-RNN on aperiodic activities is attributed to its
structural modeling of human motion. While the overall body motion can be
aperiodic, but specific parts of the body move in an (almost) periodic manner.
S-RNN models each body part separately with nodeRNNs and captures interactions
between  them with edgeRNNs in order to produce a coherent human motion. On
periodic activities such as walking, all methods forecast acceptable human
motion. S-RNN produces both realistic and smooth human motion while the motion
generated by ERD was realistic but not very smooth. The motions forecasted by
LSTM-3LR were not diverse, and on many test examples it converges to a mean
walking pose (\todo{Supplementary videos}).



\noindent \textbf{Quantitative evaluation} of motion forecasting is tricky due
to stochasticity in human motion. For this reason most of the previous works
present qualitative results. We follow the evaluation metric of Fragkiadaki et
al.~\citep{Fragkiadaki15} and present the 3D angle error between the forecasted
mocap frame and the ground truth in Table~\ref{tab:3derror}.  In short-term
motion generation S-RNN outperforms both LSTM-3LR and ERD on walking, eating,
smoking and discussion activities.  This shows while producing realistic human
motion, S-RNN also mimics the ground truth in the short-term. On the other hand,
while (qualitatively) ERD models human motion better than LSTM-3LR, it does not
	perform as well the in short-term prediction. Fragkiadaki et
	al.~\citep{Fragkiadaki15} also noted this trade-off between ERD and
	LSTM-3LR. Therefore S-RNN gives the best of both world by mimicking  the
	ground truth in the short-term and generating human like motion in the
	long term. Due to stochasticity in human motion, long-term forecasts
	($>$ 500ms) can significantly differ from the ground truth but they can
	still depict human-like motion. For this reason, the long-term forecast
	numbers in Table~\ref{tab:3derror} are not a fair representative of
	algorithms modeling capabilities. We further observe that discussion
	activity is one of the most challenging aperiodic activity on which the
	algorithms did not perform very well. 


In this section we present several insights into our S-RNN architecture. In
particular we visualize activations of S-RNN memory cells in response to several
semantic concepts. We also study the converge of our architecture on training
and test set with iterations. Since each RNN in our architecture is related to a
semantic concept this gives us flexibility to create hybrid models by
hand-picking  nodeRNNs and edgeRNNs from different S-RNN and combining to form a
new S-RNN architecture. We present these studies on mocap data set.  


\textbf{Visualization of memory units.} The RNNs in our architecture represent
different semantic concepts from the st-graph. In order to understand if they
represent any semantically meaningful concepts  we visualize the memory cells of
nodeRNNs for mocap generation on H3.6m data set. The structural nature of our
architecture allows us to study each body part separately thereby factoring an
overall complex motion into simpler semantic concepts. We found that a
particular cell in the nodeRNN modeling the leg \textit{learns the semantic
concept of walking}. The cell fires positive (red color) whenever the subject
takes a step forward, and fires negative (blue color) when the leg moves
backward. In Figure~\ref{fig:memory_cell} (left) we visualize the cell
activations of the nodeRNN modeling the leg. We observe that as the subject
walks the same cell fires alternatively for left leg and right leg. Since the
subject walks in a circle where right leg steps are longer than the left leg, we
observe the activations for right leg stays high (red) for a longer period. We
observed a similar behaviour in the nodeRNN modeling the arm. A particular cell
learns the semantic concept of \textit{moving hand close to face}. In
Figure~\ref{fig:memory_cell} (right) we visualize this cell for different
sequences of eating and smoking activities. We observe that the cell fires
whenever the subject moves hand close	 to the face.
Figure~\ref{fig:memory_cell} visualizes the cell for sequences with different
number of movements of hand to the face and with varying speeds. 


\textbf{Generating hybrid human motion.} Our architecture is structural in
nature where each RNN has a semantic meaning. This gives us the flexibility of
training multiple S-RNN architectures on varying motion styles, and then
swapping RNNs among them in order to create a novel S-RNN architecture. In order
to demonstrate novel walking styles we train S-RNN with different nodeRNNs for
left leg and right leg (i.e. assigning different colors to left leg and right
leg nodes in Figure~\ref{fig:stgraphexp}\rc{a}). We train two such S-RNN
architectures, one with down sampling H3.6m by two (at 100Hz) and other without
down sampling (at 200Hz). The architecture without down sampling generates
slower human motions  than the architecture with down sampling.  We then replace
the left leg of the S-RNN generating faster motions with the S-RNN generating
slower motions. The resulting S-RNN produces a walking motion where the human
jumps on left leg while moving forward as shown in Figure~\ref{fig:loss} (Left).
This is an expected outcome because the left leg moves at half the speed of the
right leg. The only way to keep up with this motion style is to take forward
jumps on the left leg.\footnote{Imagine your motion forward if someone holds
your right leg and runs forward!} Models such as ERD~\citep{Fragkiadaki15} which
train a single architecture does not offer this kind of flexibility. 

\textbf{S-RNN convergence and complexity.} We study the convergence of S-RNN by
examining its train and test error with iterations. In Figure~\ref{fig:loss}
(Right) we plot the train and test error of S-RNN and ERD for modeling human
motion. Both methods give similar training error, however S-RNN converges to a
smaller test error for next step prediction. Therefore S-RNN generalizes better
on test set. 

We discuss two aspects of S-RNN complexity: (i) complexity of forward-pass; and
(ii) the model size (i.e. the number of parameters). For a given st-graph, the
model size of S-RNN depends of the number of \textit{distinct} node and edge
factors in the graph (Section~\ref{sec:stgraph}). In context-rich applications,
the number of distinct factors is limited by the number of semantically similar
nodes. For this reason even for large st-graphs the resulting S-RNN can be
compact if the number of \textit{semantically similar} nodes are few -- which is
the case in many applications we encounter. The complexity of forward-pass
depends on the number of nodeRNNs and edgeRNNs. Since the forward-pass through
all edgeRNNs and nodeRNNs can be done in parallel, in practice, the forward-pass
complexity effectively depends only  on cascade of two neural networks (edgeRNN
followed by nodeRNN). To summarize, the overall computational complexity of
S-RNN depends on the number of semantically similar nodes and edges in the
graph, and not as much on the size of the st-graph. 

\fi

\iffalse
In this section we present S-RNN for the modeling of context rich human
activities. We consider the activities in CAD-120~\citep{Koppula13b} data set in
which human subjects perform household chores in unstructured environments. In
each activity (e.g. eating) a human subject interacts with several objects and
performs a sequence of sub-activities (e.g. moving, drinking etc.) in order to
complete the overall task. Koppula et al.~\citep{Koppula13,Koppula13b}
represents the rich spatial and temporal interactions between the human and
objects with the st-graph shown in Figure~\ref{fig:stgraphexp}\rc{b}. At each
time step the st-graph represents the sub-activity being performed and
affordances of the objects in the environment  (e.g., graspable, reachable
etc.). The human node is labeled with the sub-activity and object nodes are
labeled with the objects' affordances. Having observed the st-graph upto time
$t$, the goal is to \textit{detect} the sub-activity and affordance labels at
time $t$, and also \textit{anticipate} the future labels of the time step $t+1$.
Koppula et al.~\citep{Koppula13,Koppula13b} models detection and anticipation in
a probabilistic framework with Conditional Random Fields (CRF). We use S-RNN for
this problem and compare with Koppula et al.~\citep{Koppula13,Koppula13b}. As
node and edge features, we use the features provided by Koppula et
al.~\citep{Koppula13b}.

Figure~\ref{fig:stgraph}\rc{b} shows our S-RNN architecture of the st-graph
modeling human activity (Figure~\ref{fig:stgraphexp}\rc{b}). Our S-RNN have two
nodeRNNs for modeling the human and object nodes of the st-graph, and four
edgeRNNs for modeling the interactions between the nodes connected in the
st-graph.  We model edgeRNNs with one layer LSTM of size 128. The high-level
representations from edgeRNNs goes into the nodeRNNs which are modeled with an
LSTM(256)-softmax($\cdot$). The size of softmax is 10 for the nodeRNN modeling
human sub-activities and 12 for the nodeRNN modeling object
affordances.\footnote{CAD-120~\citep{Koppula13b} is annotated with 10 types of
human sub-activities and 12 types of object affordances.}  We train S-RNN for
detection by predicting the sub-activity and affordance labels of the current
time step. For anticipation we train the architecture to predict the labels of
the next time step given the observations upto the current time. We also train a
\textit{multi-task} version of S-RNN, in which we add two softmax layers to each
nodeRNN and train the architecture jointly for anticipation and detection. 

Table~\ref{tab:cad120} shows the detection and anticipation results on CAD-120
data set. S-RNN significantly improves over Koppula et al. on both
anticipation~\citep{Koppula13} and detection~\citep{Koppula13b}. Our multi-task
S-RNN improves sub-activity anticipation by 25\% and affordance anticipation
15\% over Koppula et al.~\citep{Koppula13}. On detection S-RNN is competitive to
Koppula et al.~\citep{Koppula13b}. This seems to be the case because temporal
modeling is more crucial in anticipation than detection. In the latter case,
many times a single frame suffices to detect the current activity and
affordance. Therefore S-RNN should be preferred to model st-graphs when long
temporal context is of importance to the application. Furthermore, training
S-RNN in multi-task manner on average improves the performance over S-RNN
trained disjointly. 
\fi


\textbf{Visualization of memory cells.} The RNNs in our architecture carry
semantic meanings, e.g. nodeRNNs represent different body parts.  This allows us
to study each body part separately and factor an overall complex motion into
simpler semantic concepts. In Figure~\ref{fig:memory_cell} (left) we visualize
the memory cell that \textit{learns the semantic concept of walking}. It belongs
to the nodeRNN modeling the leg. The cell fires positive (red color) on the
forward movement of leg and fires negative (blue color) on the backward
movement. So as the subject walks the cell alternates between positive and
negative activations. The cell activations for the right leg and left leg are
mutually exclusive, i.e. when the right leg has positive activation (forward)
then the left leg has negative activation (backward) and vice-versa.
Furthermore, the activations for the right leg stays high for a longer period
because the subject moves in a circle with longer forward steps with right leg.
Similarly, a cell in the nodeRNN modeling the arm, \textit{learns the semantic
concept of moving hand close to the face} as shown in
Figure~\ref{fig:memory_cell} (right). The same cell fires whenever the subject
moves the hand closer to the face, say for eating or smoking. The cell remains
active only as long as the hand stays close to the face. In
Figure~\ref{fig:memory_cell} (right) we show the same cell on different
activities and with varying number of movements of hand to the face.

\textbf{Generating hybrid human motion.} We now demonstrate benefit of our
modular architecture that enables generating novel motions which are not in the
data set. Such modularity is of interest and has been explored to generate
diverse motions~\citep{Taylor09}. The structural nature of our architecture
allows exchanging  RNNs across S-RNN architectures trained on different motion
styles. This creates a novel S-RNN model which depicts a new motion style. We
demonstrate this by creating a novel S-RNN model which generates a hybrid motion
of a \textit{human jumping forward on one leg}, as shown in
Figure~\ref{fig:loss} (Left). First, we train S-RNN architectures with different
nodeRNNs for the right and left leg (i.e. assigning different colors to left leg
and right leg nodes in Figure~\ref{fig:stgraphexp}\rc{a}). We train two such
S-RNN architectures, one with down sampling H3.6m by two (at 100Hz) and other
without down sampling (at 200Hz). The S-RNN trained without down sampling the
data generates slower human motions  than the S-RNN trained on down sampled
data. We replace the left leg of the S-RNN generating faster motions with the
left leg of S-RNN generating slower motions. The resulting S-RNN produces a
walking motion where the human jumps forward on left leg as shown in
Figure~\ref{fig:loss} (Left). This is an expected outcome because the left leg
moves at half the speed of the right leg. The only way to keep up with this
motion style is to take forward jumps on the left leg.\footnote{Imagine your
motion forward if someone holds your right leg and runs forward!} Models such as
ERD~\citep{Fragkiadaki15} which train a single architecture does not offer this
kind of flexibility.




We discuss two aspects of S-RNN complexity: (i) complexity of forward-pass; and
(ii) the model size (i.e. the number of parameters). For a given st-graph, the
model size of S-RNN depends of the number of \textit{distinct} node and edge
factors in the graph (Section~\ref{sec:stgraph}). In context-rich applications,
the number of distinct factors is limited by the number of semantically similar
nodes. For this reason even for large st-graphs the resulting S-RNN can be
compact if the number of \textit{semantically similar} nodes are few -- which is
the case in many applications we encounter. The complexity of forward-pass
depends on the number of nodeRNNs and edgeRNNs. Since the forward-pass through
all edgeRNNs and nodeRNNs can be done in parallel, in practice, the forward-pass
complexity effectively depends only  on cascade of two neural networks (edgeRNN
followed by nodeRNN). %To summarize, the overall computational complexity of
S-RNN depends on the number of semantically similar nodes and edges in the
graph, and not as much on the size of the st-graph.




As our third application we present S-RNN for anticipation of driving maneuvers
several seconds before the manuvers happen. An example include anticipation of a
future lane change maneuver several seconds before the wheel touches the lane
markings. Manuever anticipation requires spatial and temporal reasoning of the
driver, and the observations from the 	sensors inside and outside of the car.
Jain et al.~\citep{Jain15} modeled the interactions between the observations and
the driver with a spatio-temporal graph shown in
Figure~\ref{fig:stgraphexp}\rc{c}. The st-graph have three nodes representing
the observations outside the vehicle (eg. the road features), the driver's
maneuvers, and the observations inside the vehicle (eg. the driver's facial
features).	 In particular Jain et al.~\citep{Jain15} modeled the st-graph
in a probabilistic framework with a Bayesian network and their model is called
AIO-HMM. 

We model the st-graph shown in Figure~\ref{fig:stgraphexp}c with S-RNN
architecture. Our architecture consists of a nodeRNN for the driver node and two
edgeRNNs which model the interactions between the driver and the observations
inside and outside the vehicle. The driver node in the st-graph is labeled with
the future maneuver. The nodes for the outside and inside observations do not
carry any labels and therefore not modeled with nodeRNNs. Our edgeRNN networks
have a single layer LSTM of size 64 and they output high-level representations
of the edge features. The architecture of the nodeRNN is RNN(64)-softmax(5)
where the RNN layer fuses the representations from edgeRNNs. The output of
nodeRNN is softmax probabilities of the following five maneuvers: \{\textit{Left
lane change, right lane change, left turn, right turn, straight driving}\}. 

We train our S-RNN on the features provided by Jain et al.~\citep{Jain15} on
their 1100 miles of natural driving data set. The features represent the context
outside the vehicle such as the lane information, and the context inside the
vehicle such as the driver's face. 	The data set is annotated with 700
events containing 274 lane changes, 131 turns, and 295 randomly sampled
instances of driving straight. The algorithms are evaluated on their precision
and recall in anticipating maneuvers under the following three prediction
settings: (i) Lane change: algorithms only anticipate lane changes. This setting
is relevant for freeway driving; (ii) Turns: algorithms only anticipate turns;
and (iii) All maneuvers: algorithms anticipate all five maneuvers.
Table~\ref{tab:maneuver} shows the performance of different algorithms on this
task. Time-to-maneuver is the interval between the time of algorithm's
prediction and the start of the maneuver. S-RNN performs better than the
previous state-of-the-art AIO-HMM~\citep{Jain15} in every setting. It improves
precision  by 5\% and recall by 4\% when predicting all five maneuvers. The
table also shows that the performance decreases if we do not use edgeRNNs and
simply feed the concatenation of edge features into the nodeRNN. This emphasizes
the importance of edgeRNNs and the need for separately modeling different kinds
of edge interactions.


==> intro_backup.tex <==
\section{Introduction}
\begin{figure}[t]
\centering
\includegraphics[width=.9\linewidth]{../Figs/intro_fig.pdf}
\caption{\textbf{From st-graph to S-RNN.} \textbf{(Bottom)} Shows a human microwaving food. Modeling such activities requires both spatial and temporal reasoning. \textbf{(Middle)} St-graph capturing spatial and temporal interactions between the human and the objects. \textbf{(Top)} Schematic representation of our structural-RNN architecture. It captures the structure and interactions of the st-graph.}
\label{fig:pullfig}
\end{figure}


The world we live in is inherently structured. It is comprised of components that interact with each other in space and time, leading to a spatio-temporal composition. Utilizing the structure in a problem allows practitioners to inject their high-level knowledge in the learning framework. This has been the incentive for many efforts in computer vision and machine learning, such as Logic Networks~\cite{Richardson06}, Graphical Models~\cite{Koller09}, or Structured SVMs~\cite{Joachims09}, just to name a few. Modeling structural interactions that span over space and time is of particular interest to computer vision and robotics communities. Primarily, many real world interactions between humans and environment are inherently spatial and temporal (\textit{spatio-temporal}) in nature. For example, during a cooking activity humans interact with multiple objects both in space (at a given time instant) and through time. Similarly, parts of human body (arms, legs etc.) interact with each other to generate physically realizable motions such as walking.   Hence the ability to learn expressive (\textit{deep}) architectures for spatial and temporal reasoning will help many applications.  In this work, we propose a generic approach for learning  deep neural networks (DNN) with expressive structures for spatio-temporal problems. 

The notable success of DNN has proven their capability in end-to-end feature learning and labeling tasks~\cite{Zeiler14,Zheng15,X}. However, the deep architectures we commonly use lack a high-level structure which could benefit  spatio-temporal tasks. For example, it is not yet clear how to design deep architectures to capture interactions between multiple entities (say objects, body parts etc.) over both space and time. Spatio-temporal graphs (st-graph) are a popular~\citep{Koppula15,Brendel11,X} general tool for capturing high-level intuitions about a problem in space and time. Figure~\ref{fig:pullfig} (bottom \& middle) shows an example of human activity and its st-graph.   The nodes of the graph represent entities we care about such as humans, their body parts, objects etc., and edges represent the spatio-temporal interactions.  Augmenting such spatio-temporal structures with end-to-end learning capability of deep neural networks leads to a powerful tool that has the best of both worlds. We propose a method for this purpose, that is applicable to problems which can be formulated as st-graph, as defined in Section~\ref{sec:srnn}. As a result, we enable practitioners to express their high-level intuition as st-graphs and learn DNN with expressive structures using our method.

Our approach is a {generic} one that can transform an arbitrary st-graph into a feedforward Recurrent Neural Network (RNN) ensemble that is fully differentiable. Furthermore, we provide a more principled way for building structures of DNN than existing similar works~\citep{Du15,Byeon15,Chen15}, as the involved steps are well defined. In high-level steps, given an arbitrary st-graph, we first roll it out in time and decompose it into a set of contributing factor components. We then represent each of the factor components using a RNN. The key lies in capturing the structure of the st-graph by establishing connections between RNNs. The result in an ensemble of neural networks that is equivalent to the provided st-graph in terms of input, output, and spatio-temporal relationships. We refer to the resulting architecture as structural-RNN (``S-RNN''). It is {end-to-end trainable} since the formed RNN ensemble is feedforward and fully differentiable. This is of particular importance as it allows training the entire system at once without the need of any multi-state independent training.

%to multistage independent training of the components.

S-RNN is an expressive structure of multiple interconnected RNNs. Figure~\ref{fig:pullfig} (top) shows a schematic representation of S-RNN. Its structure is tied to the underlying st-graph. S-RNN consists of two types of RNNs, one that models the nodes in the st-graph and the other that models the interactions between the nodes connected in the st-graph. We will show that S-RNN architecture is scalable, as the number of parameters sub-linearly increases with an increase in the number of nodes/edges in the input st-graph. S-RNN is also modular as it allows easy manipulations due to having an underlying structure (e.g., we will experimentally show forming a feasible hybrid human by mixing parts of different subjects). The code of the entire frameworks that accepts a st-graph as the input and yields the output RNN ensemble is available at the following URL.


Even though there has been several recent efforts towards solving problems through mixing a set of RNNs, they are almost unanimously task-specific~\citep{Du15,Byeon15,Chen15}. This work is the first to provide a generic principled tool for transforming any problem that can be cast as a st-graph into an end-to-end trainable RNN ensemble. We evaluated the proposed approach on a diverse set of spatio-temporal problems (human pose modeling and forecasting, human-object interaction, and driver decision making), and show it consistently outperforms the state of the art by a large margin. The rest of the paper is organized as follows. In Section~\ref{sec:srnn} we describe the procedure for building and training S-RNN architectures. In Section~\ref{sec:experiment} we thoroughly demonstrate S-RNN on context-rich spatio-temporal problems. We also visualize the memory cells of S-RNN architecture, and study its modularity, complexity and convergence properties.

\iffalse
The world we live in is inherently structured. It is comprised of components that have individual functions yet interact with each other in space and time, leading to a fundamental spatio-temporal composition. Utilizing such a structure has been the incentive for many efforts in computer vision and machine learning, such as Logic Networks~\cite{ln}, Graphical Models~\cite{gm}, or Structured SVMs~\cite{ssvm}, just to name a few. By definition, a structured approach allows practitioners to inject their high-level knowledge in the learning framework. Besides performing predictions in a more natural way, this approach has additional crucial advantages such as enabling high-level manipulations; a component of the structure can be modified without undermining the rest of the components and their learned models. This also allows for transferring information of component across different environments without the need to learning everything from scratch.

The notable success of artificial neural networks at numerous tasks has proven their considerable capability in end-to-end learning. However, they lack a high-level structure though they have been shown to be successful at low-level feature learning~\cite{cnnvisual}. Augmenting a structured approach with end-to-end learning capability of deep neural networks leads to a powerful tool that has the best of both worlds. We propose a method for this purpose, that is applicable to largely any problem which can be formulated as a flexible high-level spatio-temporal graph,as defined in sec.~\ref{fig:strnn}.


Spatio-temporal graphs (st-graph) are a popular~\cite{stg} general tool for capturing high-level intuitions about a problem in space and time. They allow defining a set of components and their interaction in both spatial and temporal domain. In this paper, we propose a \underline{generic}, \underline{principled}, and \underline{comprehensive} method that can transform an arbitrary st-graph into a feedforward RNN ensemble that is fully differentiable, and consequently, \underline{end-to-end trainable}. 
In high-level steps, given an arbitrary st-graph, we first roll it out in time and decompose it into a set of contributing factor components. We then represent each of the factor components using a RNN. This leads to a feedforward ensemble of RNNs that is equivalent to the provided st-graph in terms of input, output, and spatio-temporal relationships. 

The proposed procedure is fundamentally more \underline{principled} than existing similar works, as the involved steps are well defined. The resulting architecture is \underline{end-to-end trainable} since the formed RNN ensemble is feedforward and fully differentiable. This is of particular importance as it allows training the entire system at once without the need to multistage independent training of the components. The approach is \underline{generic} since it does not impose any constraint on the configuration of the input st-graph. It is \underline{comprehensive} and high capacity in learning since each of the discovered factors are represented using a separate RNN; more specifically, there is one set of RNNs designated for encoding nodes’ individual states in time, one set for encoding spatio-temporal relationships among nodes, and one set for consolidating the individual and spatio-temporal states of nodes and generating the final output. We will show that this architecture is scalable as the number of parameter sublinearly increases with an increase in the number of nodes/edges in the input st-graph. It also allows easy high-level manipulations due to having an underlying structure (e.g., we will experimentally show forming a feasible hybrid human by mixing parts of different subjects). The code of the entire frameworks that accepts a st-graph as the input and yields the output RNN ensemble is available at the following github repository [URL].


Practitioners dealing with these problems capture the structure with spatio-temporal graphs (``st-graphs'')~\citep{Koppula15,Brendel11,X} (Section~\ref{sec:stgraph}).

Augmenting spatio-temporal reasoning with end-to-end learning capability of DNN leads to a powerful tool that has the best of both worlds.  We propose a method for this purpose, that is applicable to problems which can be formulated as a high-level spatio-temporal graphs (``st-graphs). , as defined in Section~\ref{fig:strnn}. As a result, we enable practitioners to express their intuition as st-graphs and then learn deep neural networks with expressive structures using our method.

The notable success of deep neural networks has proven their capability in end-to-end learning. However, the deep architectures we commonly use lack a high-level structure though they have been shown to be successful at low-level feature learning and labeling tasks~\cite{Zeiler14,Zheng15,X}. On the other hand, many context-rich interactions that take place over space and time have an inherent structure. These structures can be ``intuitively'' represented as spatio-temporal graphs (``st-graphs'')~\citep{Koppula15,Brendel11,X} (Section~\ref{sec:stgraph}). The nodes of the graph represent entities that we care about such as humans, their body parts, objects, environment etc., and the edges represent the interactions. Augmenting spatio-temporal structures with end-to-end learning capability of deep neural networks leads to a powerful tool that has the best of both worlds. We propose a method for this purpose, that is applicable to problems which can be formulated as a high-level st-graph, as defined in Section~\ref{fig:strnn}. As a result, we enable practitioners to express their intuition as st-graphs and then learn deep neural networks with expressive structures using our method.

%S-RNN is an expressive modular architecture. 
S-RNN is an expressive structure of multiple interconnected deep neural networks (RNNs). Its structure is tied to the underlying st-graph. S-RNN consists of two types of RNNs, one that models the nodes in the st-graph and the other that models the interactions between the nodes connected in the st-graph. The RNNs modeling the nodes combines the information from  RNNs modeling the edges and then predict the node labels. This form of hierarchy of RNNs makes S-RNN an expressive architecture.  We will show that S-RNN architecture is scalable, as the number of parameter sub-linearly increases with an increase in the number of nodes/edges in the input st-graph. S-RNN is also modular as it allows easy manipulations due to having an underlying structure (e.g., we will experimentally show forming a feasible hybrid human by mixing parts of different subjects). The code of the entire frameworks that accepts a st-graph as the input and yields the output RNN ensemble is available at the following github repository [URL].

\fi

==> model_backup.tex <==
\section{Structural-RNN architectures}

In this section we describe our approach for building structural-RNN (``S-RNN'') architectures for spatial and temporal reasoning. Many applications that  require this form of reasoning are modeled using spatio-temporal graphs which capture our intuition about the problem. The nodes of the graph represent entities that we care about and edges represent interactions between them. In our approach we start with a spatio-temporal graph (``st-graph''), we then represent its structure using multiple RNNs which are connected in a way they collectively capture the structure in the st-graph through parameter and feature sharing. We refer the resulting architecture as structural-RNN (S-RNN) and it provides a way to learn deep architecture for problems represented as st-graph. In Section~\ref{sec:experiment} we address several  spatio-temporal problems with S-RNN.


\subsection{Preliminaries: Spatio-temporal graphs}
\label{sec:stgraph}


A spatio-temporal graph represents interaction between entities which are represented as nodes in the graph. We represent a spatio-temporal graph (``st-graph'') with $\mathcal{G}=(\mathcal{V},\mathcal{E}_S,\mathcal{E}_T)$  whose spatial structure $(\mathcal{V},\mathcal{E}_S)$ unrolls over time through its temporal edges $\mathcal{E}_T$. At each time instant $t$ the nodes of the graph $u,v \in \mcal{V}$ are connected spatially within the same segment with an undirected edge $e=(u,v) \in \mcal{E}_S$. The temporal edge  $\bar{e}=(w,v) \in \mcal{E}_T$ at time $t$  connects the node $w$ at time $t$ to the node  $v$ at time $t+1$. Figure~\ref{fig:stgraph}a shows a  st-graph capturing interactions of a human with three objects during an activity.   The human/object nodes at time $t$ and $t+1$ are connected with temporal edges. The nodes in the graph can  assume discrete labels which we denote as $y_v$. The features associated with node $v$ and edges $e \in \mathcal{E}_S$ and $\bar{e} \in \mathcal{E}_T$ at time instant $t$  are $\ve{x}_v^t$, $\ve{x}_e^t$ and $\ve{x}_{\bar{e}}^t$. In human-object interaction the nodes features for example can represent the human/object pose, and edge features can represent their relative orientation. 


The parameterization of the st-graph is represented by its factor graph which has a factor $\Psi_v(y_v,\ve{x}_v)$ for each node and pairwise factors $\Psi_e(y_{e(1)},y_{e(2)},\ve{x}_e)$, $\Psi_{\bar{e}}(y_{\bar{e}(1)},y_{\bar{e}(2)},\ve{x}_{\bar{e}})$ for spatial and temporal edges. Furthermore, instead of learning a new factor for every node and edge, nodes/edges which are semantically similar can share factors. In Figure~\ref{fig:stgraph}a we show this by assigning same color to nodes/edges that share factors, for example the three object nodes share the node factor .This reduces the effective number of factors that needs to be learned. On this basis, the nodes and edges are partitioned into \textit{templates}  $\mcal{C}_V=\{V_1,..,V_P\}$, $\mcal{C}_E=\{E_1,..,E_M\}$, and $\mcal{C}_{\bar{E}}=\{\bar{E}_1,..,\bar{E}_N\}$ where $V_p$ is a set of nodes, and $E_m$ and $\bar{E}_n$ are sets of spatial and temporal edges such that nodes/edges within a set share factors. We denote the shared factors as $\{\Psi_{V_1},..,\Psi_{V_P}\}$, $\{\Psi_{E_1},..,\Psi_{E_M}\}$, and $\{\Psi_{\bar{E}_1},..,\Psi_{\bar{E}_N}\}$. So in all there are $P$, $M$, and $N$ distinct node factors, spatial edge factors, and temporal edge factors respectively. The function evaluated by the spatio-temporal graph for a given assignment of labels and features is a product of all the factors

\iffalse
:
\begin{align}
\nonumber \Psi(\ve{x},\ve{y})  = \prod_{t=1}^T  \left (\prod_{V_p \in C_V}\prod_{\Psi_v \in V_p} \Psi_{V_p}(y_v^t,\ve{x}_v^t;\theta_{V_p})\right) &\times \\
\nonumber \left (\prod_{E_m \in C_E }\prod_{\Psi_e \in E_m} \Psi_{E_m}(y_{e(1)}^t,y_{e(2)}^t,\ve{x}_e^t;\theta_{E_m})\right)&\times\\
 \left (\prod_{E_n \in C_{\bar{E}} }\prod_{\Psi_{\bar{e}} \in E_n} \Psi_{E_n}(y_{\bar{e}(1)}^t,y_{\bar{e}(2)}^t,\ve{x}_{\bar{e}}^t;\theta_{E_n})\right)&
\end{align}
\fi


\noindent \textbf{Neighbor factors:} We define node factor $\Psi_{V_p}$ and edge factor $\Psi_{E_m}$ as \textit{neighbors} if there exist a node $v \in V_p$ and its edge $(u,v) \in {E}_m$. Similarly node factor $\Psi_{V_p}$ and temporal edge factor $\Psi_{\bar{E}_n}$ are defined as neighbors. 

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{../Figs/stgraph.pdf}
\label{fig:stgraph2}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{../Figs/dra_small.pdf}
\caption{\textbf{An example of structural-RNN architecture.} \textbf{(a)} Spatio-temporal shows the interaction of a human with three objects during an activity. The graph unrolls over time through the directed edges. Nodes with same color share node factors and edges with same color share edge factors. The graph is therefore parameterized with two factors for nodes $\{\Psi_{V_1},\Psi_{V_2}\}$, spatial edges $\{\Psi_{E_1},\Psi_{E_2}\}$, and temporal edges $\{\Psi_{\bar{E}_1},\Psi_{\bar{E}_2}\}$. \textbf{(b)} Structural-RNN architecture have six interconnected RNNs -- one RNN for each factor. EdgeRNNs and nodeRNNs are connected to form a bipartite graph. In this example parameter sharing between human and object nodes happen through edgeRNN $\ve{R}_{E_1}$. \textbf{(c)} The forward-pass for human node $v$ involve RNNs $\ve{R}_{E_1}$, $\ve{R}_{\bar{E}_1}$ and $\ve{R}_{V_1}$. Input features into edgeRNN $\ve{R}_{E_1}$ is sum of human-object edge features $x_{v,u}$, $x_{v,o}$, $x_{v,w}$. \textbf{(d)} The forward-pass for object node $o$ involve RNNs $\ve{R}_{E_1}$, $\ve{R}_{{E}_2}$, $\ve{R}_{\bar{E}_2}$ and $\ve{R}_{V_2}$. This time the edgeRNN $\ve{R}_{E_1}$ only processes the edge feature $x_{v,o}$. Therefore edgeRNN $\ve{R}_{E_1}$ processes different linear combinations of the human-object edge features depending on the node being forward-passed. This way structural-RNN performs feature sharing. }
\label{fig:stgraph}
\end{figure*}


\subsection{Structural RNN architecture}
We now present our structural-RNN (S-RNN) architecture to represent the spatio-temporal graph described in the previous section. Our architecture consists of multiple RNNs which are connected in a way that the overall architecture captures the structure of the st-graph. Our main contribution lies in constructively building a structural-RNN architecture in which the RNNs and the connections between them are semantically related to the underlying spatio-temporal graph. This allows us, and will enable practitioners, to learn expressive deep architectures for problems that are represented as spatio-temporal graphs. 

In spatio-temporal graphs at each time step the node factor $\Psi_{V_p}$ and edge factors $\Psi_{E_m}$, $\Psi_{\bar{E}_n}$ observe node and edge features and perform some computation on those features. Our S-RNN architecture parameterizes the node factors and edge factors of the st-graph with RNNs. We refer the RNNs obtained from node factors as nodeRNNs and the RNNs obtained from edge factors as edgeRNNs.  The structure of the st-graph is captured through connections between the edgeRNNs and nodeRNNs. Each edgeRNN handles a specific kind of semantic interaction between nodes of the st-graph, and each nodeRNN combines the outputs of the edgeRNNs it is connected to and predicts the node labels.  The resulting architecture is called the structural-RNN.  


We denote the RNNs corresponding to factors $\Psi_{V_p}$, $\Psi_{E_m}$, and $\Psi_{\bar{E}_n}$ as  $\ve{R}_{V_p}$, $\ve{R}_{E_m}$, and $\ve{R}_{\bar{E}_n}$ respectively. The edgeRNNs and nodeRNNs are connected to form a bipartite graph. Figure~\ref{fig:stgraph}b shows the S-RNN for the human activity represented by the st-graph shown in  Figure~\ref{fig:stgraph}a. The edgeRNN $\ve{R}_{E_m}$ (or $\ve{R}_{\bar{E}_n}$) is connected to the nodeRNN $\ve{R}_{V_p}$ \textit{iff} the factors $\Psi_{E_m}$ (or $\Psi_{\bar{E}_n}$)  and $\Psi_{V_p}$ are \textit{neighbors} in the st-graph. The key insight in connecting edgeRNNs and nodeRNNs is to appropriately fuse the node and edge features. In order to predict the label of node $v \in V_p$ the edgeRNNs first process the edge features on the edges connected to the node. The nodeRNN $\ve{R}_{V_p}$ then combines the outputs from edgeRNNs and predicts the label of the node. This is in contrast to the parametrization of the st-graph discussed in Section~\ref{sec:stgraph} where the node and edge factors only interact through product (or through summations in log-space). In the following section we explain the inputs and outputs of RNNs, and the training procedure.


\subsection{Training structural RNN architecture}

In order to train the S-RNN architecture, for each node of the st-graph the edge and node features associated with the node are fed into the architecture.  In the forward-pass through the architecture for node $v \in V_p$, the input into edgeRNN $\ve{R}_{E_m}$ (and $\ve{R}_{\bar{E}_n}$) are the features on the edges $e \in E_m$ (and $e \in \bar{E}_n$) connected to node $v$. The output of edgeRNNs are high-level representations of the edge features.  The nodeRNN $\ve{R}_{V_p}$ concatenates the node feature with the high-level representations from the edgeRNNs and predicts the node label. At the time of training, the errors in prediction are back-propagated through the nodeRNN and edgeRNNs involved during the forward-pass. In this way our architecture non-linearly combines the node and edge features associated with the node.  Figure~\ref{fig:stgraph}c shows the forward-pass through S-RNN for human node. The edgeRNNs modeling the human-object interaction and human-human temporal interaction process the edge features connected to the human node. Since the human node is connected to three objects, the human-object edge features are accumulated and then fed into the edgeRNN as a single input vector. The nodeRNN modeling the human node concatenates the human node features with the high-level representations from edgeRNNs and outputs the node label (i.e. human activity).

\textbf{Parameter and feature sharing.} An important aspect of S-RNN lies in sharing of parameters and features across node labels. Sharing happens through the edgeRNNs which are connected to multiple nodeRNNs in the bipartite graph. For example in Figure~\ref{fig:stgraph}b the edgeRNN $\ve{R}_{E_1}$ modeling the human-object interaction is connected to both the human and object nodeRNNs. Such edgeRNNs capture the interaction between the labels, and during training their parameters gets updated through back-propagated gradients from multiple nodeRNNs they are connected to. The edge features into such edgeRNNs further captures the structure of the st-graph. This is depicted in Figure~\ref{fig:stgraph} (c \& d) where the edgeRNN $\ve{R}_{E_1}$ processes different linear combinations of the human-object edge features. Thus sharing parameters and features allows S-RNN to model the structure of the st-graph and learn interactions between the output labels.

==> supplementary_tech.tex <==
\subsection{Old writeup}
Our goal is to represent the spatio-temporal graph described above with a deep learning architecture.  We approach this problem by parameterizing the node and edge factors of the spatio-temporal graph with Recurrent Neural Networks (RNNs).  We refer the RNNs obtained in this manner as nodeRNNs and edgeRNNs respectively. Our final structural-RNN architecture captures the structure of the spatio-temporal graph through connections between the edgeRNNs and nodeRNNs. Each edgeRNN in our architecture handles a specific kind of interaction between nodes, and each nodeRNN combines the outputs of edgeRNNs it is connected to and predicts the node labels. The key insight in connecting edgeRNNs to nodeRNNs is to appropriately combine and edge and node observations for every node before predicting the labels.

In order to capture the structure of the spatio-temporal graph we connect the edgeRNNs and nodeRNNs to form a bipartite graph which we call the structural-RNN architecture.  Each edgeRNN in our architecture handles a specific kind of interaction between nodes, and each nodeRNN combines the outputs of edgeRNNs it is connected to and predicts the node labels. The key insight in connecting edgeRNNs to nodeRNNs is to appropriately combine and edge and node observations for every node before predicting the labels.

Our architecture begins with parameterizing shared node factors $\Psi_{V_p}$ and edge factors $\Psi_{E_m}$, $\Psi_{{\bar{E}_n}}$ with RNNs. We denote the RNN parameterization of $\Psi_{V_p}$ with $\ve{R}_{V_p}$ and refer to it as \textit{nodeRNN}. Likewise $\ve{R}_{E_m}$ and $\ve{R}_{\bar{E}_n}$ denote the \textit{edgeRNNs} associated with the edge factors $\Psi_{E_m}$ and $\Psi_{\bar{E}_n}$ respectively. Intuitively, edgeRNNs serves the purpose of representing the spatial and temporal interactions between the nodes of the spatio-temporal graph. Each edgeRNN is dedicated to handle a specific kind of node interaction. On the other hand, each nodeRNN is connected to multiple edgeRNNs and it temporally fuses their outputs to predict the node labels. The key to capturing the structure of the spatio-temporal graph lies in defining connections between the nodeRNNs and edgeRNNs in order to form a structural RNN architecture. 

We connect nodeRNNs and edgeRNNs to form a bipartite graph $\mcal{G}_{\ve{R}} = (\{\ve{R}_{E_m}\}\cup\{\ve{R}_{\bar{E}_n}\},\{\ve{R}_{{V}_p}\},\mcal{E}_R)$ such that the output of edgeRNNs is connected to the input of nodeRNNs. The key insight in establishing connections $\mcal{E}_R$ between nodeRNNs and edgeRNNs is to ensure that when  predicting the label of node $v$ (s.t. $\Psi_v \in {V_p}$) the nodeRNN $\ve{R}_{{V}_p}$ combines the outputs from all the edgeRNNs that represent edge factors $\Psi_{(u,v)}$ with node $v$.
 With this insight we connect edgeRNNs and nodeRNNs in $\mcal{G}_{\ve{R}}$ to capture the structure of the spatio-temporal graph $\mcal{G}$ as follows:
\begin{align}
\nonumber (\ve{R}_{E_m},\ve{R}_{{V}_p}) \in \mcal{E}_R \Longleftrightarrow& \exists u \in \mcal{V} \; \text{\&}\; \exists \Psi_v \in V_p\\
&\text{s.t.}\; \Psi_{(u,v)} \in E_m
\end{align}
The above equation convey that the nodeRNN $\ve{R}_{V_p}$ process the output from the edgeRNN $\ve{R}_{E_m}$ if there is a node $v$ and spatial edge $(u,v) \in \mcal{E}_S$ in the graph such that the node factor $\Psi_v \in {V_p}$ and the edge factor $\Psi_{(u,v)} \in {E_m}$. Likewise the edgeRNNs $\ve{R}_{\bar{E}_n}$ for temporal edges $\mcal{E}_T$ are connected to the nodeRNNs as follows: 
\begin{align}
\nonumber (\ve{R}_{\bar{E}_n},\ve{R}_{{V}_p}) \in \mcal{E}_R \Longleftrightarrow& \exists u' \in \mcal{V} \; \text{\&}\; \exists \Psi_v \in V_p\; \text{s.t.}\\
&\Psi_{(u',v)} \;\text{or}\;\Psi_{(v,u')}\in \bar{E}_n
\end{align}
Our structural RNN architecture is non-markovian and it allows nodeRNNs to non-linearly combine the outputs from multiple edgeRNN in order to predict the nodes' labels. This is in contrast to the parametrization of the spatio-temporal graph discussed in Section~\ref{sec:stgraph} where the node and edge factors only interact through product (or through summations in log-space). In the next section we will formally define the inputs and outputs into the edgeRNNs and nodeRNNs, and how we train the architecture end-to-end. 

\section{Training structured rnn}

So far we have discussed how we represent a spatio-temporal graph with an structural RNN architecture. In order to train the architecture we now define the inputs and outputs of edgeRNNs and nodeRNNs. During training the node labels $y_v^t$ and observations $\ve{x}_v^t$, $\ve{x}_e^t$, and $\ve{x}_{\bar{e}}^t$ are given for the time instants $t=1$ to $T$. For each node $v \in \mcal{V}$ we define sets $\mcal{S}_{v,E_m}$ and $\mcal{S}_{v,\bar{E}_n}$ of spatial edges $(u,v) \in \mcal{E}_S$ and temporal edges $(u',v) \in \mcal{{E}}_T$ such that the edge factors $\Psi_{(u,v)} \in  E_m$ and $\Psi_{(u',v)} \in  \bar{E}_n$ respectively.

\begin{align}
\mcal{S}_{v,E_m} = \{(u,v) | (u,v) \in \mcal{E}_S \; \text{\&}\; \Psi_{(u,v)} \in E_m\} \\
\mcal{S}_{v,\bar{E}_n} = \{(u',v) | (u',v) \in \mcal{E}_T \; \text{\&}\; \Psi_{(u',v)} \in \bar{E}_n\}
\end{align}
In order to predict the label of node $v$ the input into edgeRNN $\ve{R}_{E_m}$ at time $t$ is $\sum_{e \in \mcal{S}_{v,E_m}} \phi_{E_m}(\ve{x}_e^t)$, where $\phi_{E_m}$ is the feature function of the edge factor $\Psi_{E_m}$. If the set $\mcal{S}_{v,E_m}$ is empty then the input into edgeRNN $\ve{R}_{E_m}$ is a vector of $\ve{0}$'s. Similarly the input into edgeRNN  $\ve{R}_{\bar{E}_n}$ at time $t$ is $\sum_{e \in \mcal{S}_{v,\bar{E}_n}} \phi_{\bar{E}_n}(\ve{x}_{\bar{e}}^t)$, where $\phi_{\bar{E}_n}$ is the feature function of the edge factor $\Psi_{\bar{E}_n}$. The output of edgeRNNs $\ve{R}_{E_m}$ and $\ve{R}_{\bar{E}_n}$ at each time step $t$ are high-level representations which we denote as $\ve{h}_{E_m}^t$ and $\ve{h}_{\bar{E}_n}^t$ respectively. In this way edgeRNNs model the interactions of node $v$ with its adjacent nodes. Furthermore each edgeRNN is dedicated to model a specific kind of interaction between nodes. By parameterizing edge factors with Recurrent Neural Networks and Long Short-Term Memory (LSTM) units we allow our architecture  to model the time evolving nature of interactions between the node $v$ and its neighbouring nodes. 

The label of node $v$ where $\Psi_v \in V_p$ is predicted by the nodeRNN $\Psi_{V_p}$ which combines the high-level representations from edgeRNNs it is connected to in the bipartite graph $\mcal{G}_{\ve{R}}$. At time step $t$ the input into the nodeRNN $\Psi_{V_p}$ is  concatenation of: (i) the high-level representations $\ve{h}_{E_m}^t$ and $\ve{h}_{\bar{E}_n}^t$ from edgeRNNs such that $(\ve{R}_{E_m},\ve{R}_{{V}_p}) \in \mcal{E}_R$ and $(\ve{R}_{\bar{E}_n},\ve{R}_{{V}_p}) \in \mcal{E}_R$; with (ii) the feature representation $\phi_{V_p}(\ve{x}_v^t)$ of node observation, where  $\phi_{V_p}$ is the feature function of node factor $\Psi_{V_p}$.


